Locality-aware Gaussian Compression for Fast and High-quality Rendering

We present LocoGS, a locality-aware 3D Gaussian Splatting (3DGS) framework that exploits the spatial coherence of 3D Gaussians for compact modeling of volumetric scenes. To this end, we first analyze the local coherence of 3D Gaussian attributes, and propose a novel locality-aware 3D Gaussian representation that effectively encodes locally-coherent Gaussian attributes using a neural field representation with a minimal storage requirement. On top of the novel representation, LocoGS is carefully designed with additional components such as dense initialization, an adaptive spherical harmonics bandwidth scheme and different encoding schemes for different Gaussian attributes to maximize compression performance. Experimental results demonstrate that our approach outperforms the rendering quality of existing compact Gaussian representations for representative real-world 3D datasets while achieving from 54.6$\times$ to 96.6$\times$ compressed storage size and from 2.1$\times$ to 2.4$\times$ rendering speed than 3DGS. Even our approach also demonstrates an averaged 2.4$\times$ higher rendering speed than the state-of-the-art compression method with comparable compression performance.

==> figs/main/ablation_hash.tex <==
% \begin{figure*}[!ht]
% \begin{minipage}[b]{0.45\textwidth}
%     % \vspace{+2mm}
%     \centering
%     \captionof{table}{\todo{Appendix} Ablation study on position compression. We evaluate rendering quality and storage size of position.}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{lccccc}
%         \toprule
%         Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & Size $\downarrow$ \\
%         \midrule
%         Baseline (16-bit) & 27.33 & 0.814 & 0.219 & 7.95 \\
%         + Entropy coding & 27.33 & 0.814 & 0.219 & 7.37 \\
%         + Morton sorting & 27.33 & 0.814 & 0.219 & 5.94 \\
%         + Octree codec & 27.33 & 0.814 & 0.219 & 2.80 \\
%         \bottomrule
%     \end{tabular}}
% \label{tab:ablation_octree}
% \end{minipage}\hfill
% \begin{minipage}[b]{0.53\textwidth}
%     \begin{center}
%     \includegraphics[width=\linewidth]{assets/main/hash_size.pdf}
%     \end{center}
%     \vspace{-4mm}
%     \caption{Ablation study on the hash grid size.}
%     % \vspace{-2mm}
%     \label{fig:ablation_hash}
% \end{minipage}
% \end{figure*}



% \begin{figure*}[!ht]
%     \begin{center}
%     \includegraphics[width=0.4\linewidth]{assets/main/hash_size.pdf}
%     \end{center}
% \vspace{-4mm}
% \caption{Ablation study on the hash grid size.}
% % \vspace{-2mm}
% \label{fig:ablation_hash}
% \end{figure*}


\begin{wrapfigure}{r}{0.52\textwidth}
\vspace{-6mm}
    \begin{center}
    \includegraphics[width=\linewidth]{assets/main/hash_size.pdf}
    \end{center}
\vspace{-5mm}
\caption{Ablation study on the hash grid size.}
\vspace{-4mm}
\label{fig:ablation_hash}
\end{wrapfigure}



==> figs/main/derivation.tex <==
\begin{figure*}[!ht]
\begin{center}
% \vspace{-4mm}
\includegraphics[width=0.4\linewidth]{assets/main/derivation.pdf}
\end{center}
% \vspace{-4mm}
\caption{.}
% \vspace{-4mm}
\label{fig:derivation}
\end{figure*}

==> figs/main/initialization.tex <==
\begin{figure}[!ht]%${r}{0.45\textwidth}
    % \vspace{-4mm}
    \begin{center}
    \includegraphics[width=0.45\textwidth]{assets/main/initialization.pdf}
    \end{center}
    \caption{Visualization of initial point cloud.}
    \label{fig:initialization}
\end{figure}


==> figs/main/sh_mask.tex <==
\begin{wrapfigure}{r}{0.24\textwidth}
% \vspace{-5mm}
\includegraphics[width=0.24\textwidth]{assets/main/sh_mask.pdf}
% \vspace{-4mm}
\caption{Illustration of SH bandwidth pruning.}
% \vspace{-6mm}
\end{wrapfigure}


==> figs/rebuttal/decode_rebuttal.tex <==
\begin{figure*}[t]
\begin{center}
% \vspace{-4mm}
\includegraphics[width=0.8\linewidth]{assets/rebuttal/rebuttal_decode.pdf}
\end{center}
\vspace{-4mm}
\caption{Evaluation.}
\vspace{-4mm}
\label{fig:rebuttal_decode}
\end{figure*}

==> figs/rebuttal/locality_rebuttal.tex <==
\begin{figure*}[t]
\begin{center}
% \vspace{-4mm}
\includegraphics[width=1.0\linewidth]{assets/rebuttal/local_similarity_rebuttal.pdf}
\end{center}
\vspace{-4mm}
\caption{Evaluation of the local similarity of Gaussian attributes. A histogram of local similarity according to the distance between adjacent Gaussians (top) and a chart of averaged local similarity along the distance between adjacent Gaussians (bottom).}
\vspace{-4mm}
\label{fig:rebuttal_locality}
\end{figure*}

==> figs/rebuttal/performance_rebuttal.tex <==
\begin{figure*}[t]
\begin{center}
% \vspace{-4mm}
\includegraphics[width=0.6\linewidth]{assets/rebuttal/rebuttal_performance.pdf}
\end{center}
\vspace{-2mm}
\caption{Evaluation.}
\vspace{-4mm}
\label{fig:rebuttal_performance}
\end{figure*}

==> figs/rebuttal/qual_rebuttal.tex <==
\begin{figure*}[t]
\begin{center}
% \vspace{-4mm}
\includegraphics[width=\linewidth]{assets/rebuttal/rebuttal_qual_combine.pdf}
\end{center}
\vspace{-2mm}
\caption{Qualitative results on the `bicycle' scene with averaged LPIPS for all test views and storage size on the right upper.}
\vspace{-4mm}
\label{fig:rebuttal_qual}
\end{figure*}

==> figs/rebuttal/qual_revision_rebuttal.tex <==
\begin{figure*}[t]
\begin{center}
% \vspace{-4mm}
\includegraphics[width=0.7\linewidth]{assets/rebuttal/rebuttal_qual_revision.pdf}
\end{center}
\vspace{-4mm}
\caption{Qualitative results on the `bicycle` scene with LPIPS and storage size on the right upper.}
\vspace{-4mm}
\label{fig:rebuttal_qual_revision}
\end{figure*}

==> figs/rebuttal/score_rebuttal.tex <==
% \begin{figure*}[t]
% \begin{center}
% % \vspace{-4mm}
% \includegraphics[width=0.6\linewidth]{assets/rebuttal/rebuttal_score.pdf}
% \end{center}
% \vspace{-2mm}
% \caption{Evaluation.}
% \vspace{-4mm}
% \label{fig:rebuttal_score}
% \end{figure*}

\begin{figure*}[!t]
\begin{minipage}[b]{0.75\textwidth}
    \begin{center}
    \includegraphics[width=\linewidth]{assets/rebuttal/rebuttal_score.pdf}
    \end{center}
\vspace{-2mm}
\caption{Evaluation of the rendering quality, rendering speed, and storage size (top). Evaluation of the decoding time and storage size (bottom).}
\vspace{-3.5mm}
\label{fig:rebuttal_score}
\end{minipage}\hfill
\begin{minipage}[b]{0.23\textwidth}
    \begin{center}
    \includegraphics[width=\linewidth]{assets/rebuttal/rebuttal_num.pdf}
    \end{center}
\vspace{-2mm}
\caption{Evaluation of the number of Gaussians along iterations.}
\vspace{-4mm}
\label{fig:rebuttal_num}
\end{minipage}
\end{figure*}

==> sections/main/locality.tex <==
\section{Locality-Awareness Analysis} \label{sec:locality}

We concentrate on the locality-awareness as an inductive bias to represent Gaussian attributes. Existing Gaussian representations do not employ the local information of Gaussians since they are independently parameterized with explicit attributes. Thus, we analyze the locality-awareness of Gaussians to leverage mutual local information for achieving compact Gaussian representation. Fig.~\ref{fig:local_similarity} demonstrates that Gaussians contain similar attribute values with their neighboring ones, indicating that the Gaussians follow local similarity. Therefore, we efficiently parameterize Gaussian attributes as spatial continuous signals by adopting a neural field, one of representative locality-aware representations, to achieve compact 3D Gaussian representation with reduced storage costs. In the following, we demonstrate how to construct the overall framework based on this analysis.

% We concentrate on the compactness of the neural fields as an optimal solution to alleviate the excessive storage of Gaussian attributes, which serve as a severe storage bottleneck in the current 3DGS framework. The neural fields build a coordinate-based system representing continuous signals. Accordingly, we examine the continuity of Gaussian attributes to achieve compact neural field-based Gaussian representation. Fig.~\ref{fig:local_similarity} demonstrates that each Gaussian shares similar attribute values with its neighboring ones, indicating that the Gaussian follows local similarity. Therefore, we propose a local-aware Gaussian representation by formulating Gaussian attributes as continuous signals encoded in the compact neural fields. In the following, we demonstrate how to construct the overall framework based on this analysis.



==> tables/main/SH_mask.tex <==
\begin{table}[!ht]%{r}{0.5\textwidth}
    \centering
    \caption{Ablation study on residual SH pruning.}
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lcccccc}
        \toprule
        Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & Size $\downarrow$ & FPS $\uparrow$ \\
        \midrule
        $L=3$ & 27.29 & 0.814 & 0.219 & 13.52 & 238 \\
        $L=2$ & 27.22 & 0.813 & 0.220 & 13.58 & 258 \\
        $L=1$ & 27.08 & 0.811 & 0.221 & 13.62 & 268 \\
        $L=0$ & 26.72 & 0.804 & 0.226 & 13.90 & 269 \\
        \midrule
        Ours & 27.33 & 0.814 & 0.219 & 13.83 & 270 \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:ablation_sh}
\end{table}

==> tables/main/ablation_design.tex <==
\begin{table}[!ht]
    \centering
    \caption{Ablation study on the design of the representation.}
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lcccccc}
        \toprule
        Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & Size $\downarrow$ & FPS $\uparrow$ \\
        \midrule
        w/o base scale & 27.21 & 0.807 & 0.232 & 14.88 & 231 \\
        w/o base color & 27.33 & 0.814 & 0.219 & 13.89 & 270 \\
        
        \bottomrule
    \end{tabular}
    }
    \vspace{-4mm}
    \label{tab:ablation_init}
\end{table}

==> tables/main/ablation_method.tex <==
\begin{table*}[ht]
    \centering
    \caption{Ablation study on the compression pipeline.}
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lccccc}
        \toprule
        Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & Size (MB) $\downarrow$ \\
        \midrule
        Baseline 
        & 27.47 & 0.814 & 0.221 & 50.00 \\
        + R-VQ 
        & 27.51 & 0.814 & 0.222 & 36.78 (-26.4\%) \\
        + Grid quantization
        & 27.48 & 0.814 & 0.223 & 21.03 (-57.9\%) \\
        + Entropy encoding
        & 27.48 & 0.814 & 0.223 & 18.14 (-63.7\%) \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:ablation_method}
\end{table*}

==> tables/main/comparison_mip360.tex <==
\begin{table*}[ht]
    \centering
    \caption{Evaluation on Mip-NeRF 360 dataset~\cite{barron2022mip}.}
    \resizebox{0.75\textwidth}{!}{
    \begin{tabular}{lccccc}
        \toprule
            \multirow{2}{*}{Method} &
            \multicolumn{5}{c}{Mip-NeRF 360 ~\cite{barron2022mip}} \\
            \cmidrule(lr){2-6} 
            & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$ \\
        \midrule
        3DGS~\cite{kerbl20233d}
        & 27.49 & 0.812 & 0.222 & 769.9 & 123  \\ 
        Scaffold-GS~\cite{lu2023scaffold}
        & 27.78 & 0.812 & 0.226 & 179.7 & 116 \\
        \midrule
        Compact-3DGS~\cite{lee2023compact} 
        & 27.08 & 0.798 & 0.246 & 48.88 & 135 \\
        LightGaussian~\cite{fan2023lightgaussian}
        & 26.93 & 0.800 & 0.244 & 51.13 & 216 \\
        C3DGS~\cite{niedermayr2023compressed}
        & 27.15 & 0.801 & 0.241 & 29.28 & 131 \\
        CompGS~\cite{navaneet2023compact3d} 
        & 27.03 & 0.803 & 0.238 & 85.57 & 115 \\
        EAGLES~\cite{girish2023eagles}
        & 27.13 & 0.805 & 0.239 & 71.30 & 148 \\
        HAC~\cite{chen2024hac}
        & 27.43 & 0.804 & 0.242 & 16.00 & 106 \\
        \midrule
	    Ours-Light
        &  \\
        Ours 
        & 27.48 & 0.814 & 0.223 & 18.14 & 224 \\ 
        \bottomrule
    \end{tabular}
    }
    \label{tab:comparison_tandt_db}
\end{table*}




% \begin{table*}[ht]
%     \centering
%     \caption{Evaluation on Mip-NeRF 360 dataset~\cite{barron2022mip} and Tanks and Temples dataset~\cite{knapitsch2017tanks}.}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{lcccccccccc}
%         \toprule
%             \multirow{2}{*}{Method} &
%             \multicolumn{5}{c}{Mip-NeRF 360~\cite{barron2022mip}} &
%             \multicolumn{5}{c}{Tanks and Temples~\cite{knapitsch2017tanks}} \\
%             \cmidrule(lr){2-6} \cmidrule(lr){7-11}
%             & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$
%             & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$ \\
%         \midrule
%         3DGS~\cite{kerbl20233d}
%         & 27.49 & 0.812 & 0.222 & 769.9 & 123 
%         & 23.66 & 0.845 & 0.178 & 429.5 & 176 \\
%         Scaffold-GS~\cite{lu2023scaffold} 
%         & 27.78 & 0.812 & 0.226 & 179.7 & 116
%         & 24.03 & 0.850 & 0.175 & 80.90 & 166 \\
%         \midrule
%         Compact-3DGS~\cite{lee2023compact} 
%         & 27.08 & 0.798 & 0.246 & 48.88 & 135 
%         & 23.32 & 0.831 & 0.202 & 39.40 & 201 \\
%         LightGaussian~\cite{fan2023lightgaussian} 
%         & 26.93 & 0.800 & 0.244 & 51.13 & 216  
%         & 23.32 & 0.830 & 0.204 & 30.03 & 374 \\
%         C3DGS~\cite{niedermayr2023compressed} 
%         & 27.15 & 0.801 & 0.241 & 29.28 & 131
%         & 23.47 & 0.838 & 0.188 & 18.42 & 211 \\
%         Compact3D~\cite{navaneet2023compact3d} 
%         & 27.17 & 0.808 & 0.229 & 64.93 & 115 
%         & 23.48 & 0.840 & 0.188 & 36.27 & 172 \\
%         EAGLES~\cite{girish2023eagles} 
%         & 27.13 & 0.805 & 0.239 & 71.30 & 148 
%         & 23.48 & 0.836 & 0.200 & 35.33 & 265\\
%         HAC~\cite{chen2024hac} 
%         & 27.43 & 0.804 & 0.242 &  16.0 & 106
%         & 24.16 & 0.846 & 0.187 &  8.35 & 134 \\
%         \midrule
% 	    Ours-Small \\
%         Ours \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:comparison}
% \end{table*}

% \begin{table*}[ht]
%     \centering
%     \caption{Evaluation on Deep Blending dataset~\cite{hedman2018deep}.}
%     \resizebox{0.6\textwidth}{!}{
%     \begin{tabular}{lccccc}
%         \toprule
%             \multirow{2}{*}{Method} &
%             \multicolumn{5}{c}{Deep Blending~\cite{hedman2018deep}} \\
%             \cmidrule(lr){2-6} 
%             & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$ \\
%         \midrule
%         3DGS~\cite{kerbl20233d}
%         & 29.51 & 0.900 & 0.246 & 661.0 & 135 \\ 
%         Scaffold-GS~\cite{lu2023scaffold}
%         & 30.18 & 0.905 & 0.256 & 56.13 & 268 \\
%         \midrule
%         Compact-3DGS~\cite{lee2023compact} 
%         & 29.83 & 0.901 & 0.257 & 42.91 & 191 \\
%         LightGaussian~\cite{fan2023lightgaussian}
%         & 23.35 & 0.830 & 0.204 & 30.03 & 374 \\
%         C3DGS~\cite{niedermayr2023compressed}
%         & 29.40 & 0.898 & 0.255 & 25.07 & 156 \\
%         Compact3D~\cite{navaneet2023compact3d}
%         & 29.83 & 0.901 & 0.257 & 42.91 & 124 \\
%         EAGLES~\cite{girish2023eagles}
%         & 29.89& 0.906 & 0.249 & 64.31 & 169 \\
%         HAC~\cite{chen2024hac}
%         & 29.97 & 0.903 & 0.267 & 4.78 & 238 \\
%         \midrule
% 	    Ours-Small \\
%         Ours \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:comparison_db}
% \end{table*}

==> tables/main/comparison_summary.tex <==
\begin{table*}[ht]
    \centering
    \caption{Summarized comparison to existing compact 3D Gaussian Splatting methods.}
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lccc}
        \toprule
        Method & Compactness & Rendering & High-quality \\
        \midrule
        3DGS~\cite{kerbl20233d} & \xmark & \xmark & \cmark \\
        Scaffold-GS~\cite{lu2023scaffold} & \xmark & \xmark & \cmark\\
        \midrule
        CompGS~\cite{navaneet2023compact3d} & \cmark & \xmark & \xmark \\
        Compact-3DGS~\cite{lee2023compact} & \cmark & \xmark & \xmark \\
        C3DGS~\cite{niedermayr2023compressed} & \cmark & \xmark & \xmark \\
        LightGaussian~\cite{fan2023lightgaussian} & \cmark & \cmark & \xmark \\ 
        EAGLES~\cite{girish2023eagles} & \cmark & \cmark & \xmark \\
        HAC~\cite{chen2024hac} & \cmark & \xmark & \cmark \\
        \midrule
        \rowcolor{yellow!50}Ours & \cmark & \cmark & \cmark \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:comparison_summary}
\end{table*}


% \begin{table*}[ht]
%     \centering
%     \caption{Summarized comparison to existing compact 3D Gaussian Splatting methods.}
%     \resizebox{0.5\textwidth}{!}{
%     \begin{tabular}{lcc}
%         \toprule
%         Method & Compactness & Rendering & High-quality \\
%         \midrule
%         3DGS~\cite{kerbl20233d} & \xmark & \xmark & \cmark \\
%         Scaffold-GS~\cite{lu2023scaffold} & \xmark & \xmark & \cmark\\
%         \midrule
%         CompGS~\cite{navaneet2023compact3d} & \cmark & \xmark & \xmark \\
%         Compact-3DGS~\cite{lee2023compact} & \cmark & \xmark & \xmark \\
%         C3DGS~\cite{niedermayr2023compressed} & \cmark & \xmark & \xmark \\
%         LightGaussian~\cite{fan2023lightgaussian} & \cmark & \cmark & \xmark \\ 
%         EAGLES~\cite{girish2023eagles} & \cmark & \cmark & \xmark \\
%         HAC~\cite{chen2024hac} & \cmark & \xmark & \cmark \\
%         \midrule
%         \rowcolor{yellow!50}Ours & \cmark & \cmark & \cmark \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:comparison_summary}
% \end{table*}


==> tables/main/octree_encoding.tex <==
\begin{figure*}[!ht]
\begin{minipage}[b]{0.49\textwidth}
    \centering
    \captionof{table}{Ablation study on residual SH pruning.}
    \vspace{-2mm}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccc}
        \toprule
        Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & Size $\downarrow$ & FPS $\uparrow$ \\
        \midrule
        $L=3$ & 27.29 & 0.814 & 0.219 & 13.58 & 238 \\
        $L=2$ & 27.22 & 0.813 & 0.220 & 13.64 & 258 \\
        $L=1$ & 27.08 & 0.811 & 0.221 & 13.68 & 268 \\
        $L=0$ & 26.72 & 0.804 & 0.226 & 13.96 & 269 \\
        \midrule
        Ours & 27.33 & 0.814 & 0.219 & 13.89 & 270 \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:ablation_sh}
    % \vspace{+2mm}
    \centering
    \captionof{table}{Ablation study on position compression. We evaluate rendering quality and storage size of position.}
    \vspace{+1mm}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccc}
        \toprule
        Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & Size $\downarrow$ \\
        \midrule
        Baseline (16-bit) & 27.33 & 0.814 & 0.219 & 7.95 \\
        + Entropy encoding & 27.33 & 0.814 & 0.219 & 7.37 \\
        + Morton sorting & 27.33 & 0.814 & 0.219 & 5.94 \\
        + Quantization (14-bit) & 26.90 & 0.789 & 0.235 & 4.68 \\
        \midrule
        Ours & 27.33 & 0.814 & 0.219 & 2.80 \\
        \bottomrule
    \end{tabular}}
\label{tab:ablation_octree}
\end{minipage}\hfill
\begin{minipage}[b]{0.49\textwidth}
    % \vspace{-4mm}
    \begin{center}
    \includegraphics[width=\textwidth]{assets/main/initialization_bicycle.pdf}
    \end{center}
    \vspace{-2mm}
    \caption{Visualization of the initial point cloud (upper) and rendering image (bottom).\TODO{To appendix}}
    \label{fig:initialization}
    % Octree + Uniform Q. & 26.90 & 0.789 & 0.235 & 2.77 \\
    % Octree + Log Q. & 27.33 & 0.814 & 0.219 & 3.62 \\
\end{minipage}
\end{figure*}



==> tables/rebuttal/comparison_mip360.tex <==
% \begin{table*}[ht]
%     \centering
%     \caption{Quantitative evaluation on the Mip-NeRF 360 dataset. We report the average scores of all scenes in the dataset. We highlight the \colorbox{red!35}{best score}, \colorbox{orange!35}{second-best score}, and \colorbox{yellow!35}{third-best score}.}
%     \resizebox{0.6\textwidth}{!}{
%     \begin{tabular}{lccccc}
%         \toprule
%             \multirow{2}{*}{Method} &
%             \multicolumn{5}{c}{Mip-NeRF 360} \\
%             \cmidrule(lr){2-6} 
%             & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$ \\
%         \midrule
%         CompGS
%         & 27.03 & 0.803 & \cellcolor{red!35} 0.238 & 85.57 & 115 \\
%         Compact-3DGS
%         & 27.08 & 0.798 & 0.246 & 48.88 & 135 \\
%         C3DGS
%         & \cellcolor{yellow!35} 27.15 & 0.801 & \cellcolor{yellow!35} 0.241 & \cellcolor{yellow!35} 29.28 & 131 \\
%         LightGaussian
%         & 26.93 & 0.800 & 0.244 & 51.13 & \cellcolor{yellow!35}{216} \\
%         EAGLES
%         & 27.13 & \cellcolor{orange!35} 0.805 & \cellcolor{orange!35} 0.239 & 71.30 & \cellcolor{yellow!35} 148 \\
%         HAC
%         & \cellcolor{red!35} 27.43 & 0.\cellcolor{yellow!35} 804 & 0.242 & \cellcolor{red!35}{16.00} & 106 \\
%         \midrule
%         Ours-Sparse
%         & \cellcolor{orange!35} 27.31 & \cellcolor{red!35}{0.807} & \cellcolor{red!35} 0.238 & \cellcolor{orange!35} 19.42 & \cellcolor{orange!35} 193 \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


\begin{table*}[t]
    \centering
    \caption{Quantitative evaluation. We report the average scores of all scenes in the dataset.  
    % We highlight the \colorbox{red!35}{best score}, \colorbox{orange!35}{second-best score}, and \colorbox{yellow!35}{third-best score}.
    }
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccccccccc}
        \toprule
            \multirow{2}{*}{Method} &
            \multicolumn{5}{c}{Mip-NeRF 360 (9 scenes)} &
            \multicolumn{5}{c}{Tanks and Temples (2 scenes)} &
            \multicolumn{5}{c}{Deep Blending (2 scenes)} \\
            \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
            & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$
            & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$
            & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$ \\
        \midrule
        CompGS
        & 27.03 & 0.803 & \cellcolor{red!35} 0.238 & 85.57 & 115
        & 23.36 & 0.837 & 0.193 & 49.31 & 172 
        & 29.83 & 0.903 & \cellcolor{red!35}{0.248} & 75.91 & 124 \\
        Compact-3DGS
        & 27.08 & 0.798 & 0.246 & 48.88 & 135 
        & 23.32 & 0.831 & 0.202 & 39.40 & 201 
        & 29.83 & 0.901 & 0.257 & 42.91 & 191 \\
        C3DGS
        & \cellcolor{yellow!35} 27.15 & 0.801 & \cellcolor{yellow!35} 0.241 & \cellcolor{yellow!35} 29.28 & 131 
        & 23.47 & \cellcolor{yellow!35} 0.838 & \cellcolor{yellow!35} 0.188 & \cellcolor{yellow!35} 18.42 & 211 
        & 29.40 & 0.898 & 0.255 & \cellcolor{yellow!35} 25.07 & 156 \\
        LightGaussian
        & 26.93 & 0.800 & 0.244 & 51.13 & \cellcolor{red!35}{216} 
        & 23.32 & 0.830 & 0.204 & 30.03 & \cellcolor{red!35}{374}
        & 29.09 & 0.894 & 0.262 & 45.42 & \cellcolor{red!35}{286} \\
        EAGLES
        & 27.13 & \cellcolor{orange!35} 0.805 & \cellcolor{orange!35} 0.239 & 71.30 & \cellcolor{yellow!35} 148 
        & \cellcolor{yellow!35} 23.48 & 0.836 & 0.200 & 35.33 & \cellcolor{orange!35} 265 
        & \cellcolor{yellow!35} 29.89 & \cellcolor{red!35}{0.906} & \cellcolor{orange!35} 0.249 & 64.31 & 169 \\
        HAC
        & \cellcolor{red!35} 27.43 & 0.\cellcolor{yellow!35} 804 & 0.242 & \cellcolor{red!35}{16.00} & 106 
        & \cellcolor{red!35}{24.16} & \cellcolor{red!35} 0.846 & \cellcolor{orange!35} 0.187 &  \cellcolor{red!35}{8.35} & 134 
        & \cellcolor{orange!35} 29.97 & \cellcolor{yellow!35} 0.903 & 0.267 &  \cellcolor{red!35}{4.78} & \cellcolor{orange!35} 238 \\
        \midrule
        Ours-Sparse
        & \cellcolor{orange!35} 27.31 & \cellcolor{red!35}{0.807} & \cellcolor{red!35} 0.238 & \cellcolor{orange!35} 19.42 & \cellcolor{orange!35} 193 
        & \cellcolor{orange!35} 23.79 & \cellcolor{orange!35} 0.845 & \cellcolor{red!35} 0.183 & \cellcolor{orange!35} 16.38 & \cellcolor{yellow!35} 236
        & \cellcolor{red!35}{30.16} & \cellcolor{orange!35}{0.905} & \cellcolor{yellow!35} 0.250 & \cellcolor{orange!35} 19.71 & \cellcolor{yellow!35} 213 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}


==> tables/rebuttal/comparison_octree.tex <==
% \begin{table*}[ht]
%     \centering
%     \caption{Quantitative evaluation on the Mip-NeRF 360 dataset. We report the average scores of all scenes in the dataset. We highlight the \colorbox{red!35}{best score}, \colorbox{orange!35}{second-best score}, and \colorbox{yellow!35}{third-best score}.}
%     \resizebox{0.6\textwidth}{!}{
%     \begin{tabular}{lccccc}
%         \toprule
%             \multirow{2}{*}{Method} &
%             \multicolumn{5}{c}{Mip-NeRF 360} \\
%             \cmidrule(lr){2-6} 
%             & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$ \\
%         \midrule
%         CompGS
%         & 27.03 & 0.803 & \cellcolor{red!35} 0.238 & 85.57 & 115 \\
%         Compact-3DGS
%         & 27.08 & 0.798 & 0.246 & 48.88 & 135 \\
%         C3DGS
%         & \cellcolor{yellow!35} 27.15 & 0.801 & \cellcolor{yellow!35} 0.241 & \cellcolor{yellow!35} 29.28 & 131 \\
%         LightGaussian
%         & 26.93 & 0.800 & 0.244 & 51.13 & \cellcolor{yellow!35}{216} \\
%         EAGLES
%         & 27.13 & \cellcolor{orange!35} 0.805 & \cellcolor{orange!35} 0.239 & 71.30 & \cellcolor{yellow!35} 148 \\
%         HAC
%         & \cellcolor{red!35} 27.43 & 0.\cellcolor{yellow!35} 804 & 0.242 & \cellcolor{red!35}{16.00} & 106 \\
%         \midrule
%         Ours-Sparse
%         & \cellcolor{orange!35} 27.31 & \cellcolor{red!35}{0.807} & \cellcolor{red!35} 0.238 & \cellcolor{orange!35} 19.42 & \cellcolor{orange!35} 193 \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


\begin{table*}[ht]
    \centering
    \caption{Quantitative evaluation. We report the average scores of all scenes in the dataset. We highlight the \colorbox{red!35}{best score}, \colorbox{orange!35}{second-best score}, and \colorbox{yellow!35}{third-best score}.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccccccccc}
        \toprule
            \multirow{2}{*}{Method} &
            \multicolumn{5}{c}{Mip-NeRF 360 (9 scenes)} &
            \multicolumn{5}{c}{Tanks and Temples (2 scenes)} &
            \multicolumn{5}{c}{Deep Blending (2 scenes)} \\
            \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
            & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$
            & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$
            & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$ \\
        \midrule
        CompGS
        & 27.03 & 0.803 & \cellcolor{orange!35} 0.238 & 85.57 & 115
        & 23.36 & 0.837 & 0.193 & 49.31 & 172 
        & 29.83 & 0.903 & \cellcolor{red!35}{0.248} & 75.91 & 124 \\
        Compact-3DGS
        & 27.08 & 0.798 & 0.246 & 48.88 & 135 
        & 23.32 & 0.831 & 0.202 & 39.40 & 201 
        & 29.83 & 0.901 & 0.257 & 42.91 & 191 \\
        C3DGS
        & \cellcolor{yellow!35} 27.15 & 0.801 & \cellcolor{yellow!35} 0.241 & \cellcolor{yellow!35} 29.28 & 131 
        & 23.47 & \cellcolor{yellow!35} 0.838 & \cellcolor{yellow!35} 0.188 & \cellcolor{yellow!35} 18.42 & 211 
        & 29.40 & 0.898 & 0.255 & \cellcolor{yellow!35} 25.07 & 156 \\
        LightGaussian
        & 26.93 & 0.800 & 0.244 & 51.13 & \cellcolor{red!35}{216} 
        & 23.32 & 0.830 & 0.204 & 30.03 & \cellcolor{red!35}{374}
        & 29.09 & 0.894 & 0.262 & 45.42 & \cellcolor{red!35}{286} \\
        EAGLES
        & 27.13 & \cellcolor{orange!35} 0.805 & \cellcolor{orange!35} 0.239 & 71.30 & \cellcolor{yellow!35} 148 
        & \cellcolor{yellow!35} 23.48 & 0.836 & 0.200 & 35.33 & \cellcolor{orange!35} 265 
        & \cellcolor{yellow!35} 29.89 & \cellcolor{red!35}{0.906} & \cellcolor{orange!35} 0.249 & 64.31 & 169 \\
        HAC
        & \cellcolor{red!35} 27.43 & 0.\cellcolor{yellow!35} 804 & 0.242 & \cellcolor{red!35}{16.00} & 106 
        & \cellcolor{red!35}{24.16} & \cellcolor{red!35} 0.846 & \cellcolor{orange!35} 0.187 &  \cellcolor{red!35}{8.35} & 134 
        & \cellcolor{orange!35} 29.97 & \cellcolor{yellow!35} 0.903 & 0.267 &  \cellcolor{red!35}{4.78} & \cellcolor{orange!35} 238 \\
        SOG
        & 27.09 & 0.799 & \cellcolor{red!35} 0.230 & 42.98 & 122
        & 23.52 & 0.834 & 0.188 & 42.98 & 223
        & 28.89 & 0.885 & 0.271 & 42.98 & 227 \\
        \midrule
        Ours-Sparse
        & \cellcolor{orange!35} 27.31 & \cellcolor{red!35}{0.807} & \cellcolor{orange!35} 0.238 & \cellcolor{orange!35} 19.42 & \cellcolor{orange!35} 193 
        & \cellcolor{orange!35} 23.79 & \cellcolor{orange!35} 0.845 & \cellcolor{red!35} 0.183 & \cellcolor{orange!35} 16.38 & \cellcolor{yellow!35} 236
        & \cellcolor{red!35}{30.16} & \cellcolor{orange!35}{0.905} & \cellcolor{yellow!35} 0.250 & \cellcolor{orange!35} 19.71 & \cellcolor{yellow!35} 213 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}


% \begin{table*}[ht]
%     \centering
%     \caption{Quantitative evaluation. We report the average scores of all scenes in the dataset. We highlight the \colorbox{red!35}{best score}, \colorbox{orange!35}{second-best score}, and \colorbox{yellow!35}{third-best score}.}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{lccccccccccccccc}
%         \toprule
%             \multirow{2}{*}{Method} &
%             \multicolumn{5}{c}{Mip-NeRF 360} &
%             \multicolumn{5}{c}{Tanks and Temples} &
%             \multicolumn{5}{c}{Deep Blending} \\
%             \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){11-15}
%             & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$
%             & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$
%             & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$   & Size (MB) $\downarrow$ & FPS $\uparrow$ \\
%         \midrule
%         CompGS
%         & 27.03 & 0.803 & \cellcolor{orange!35} 0.238 & 85.57 & 115
%         & 23.36 & \cellcolor{yellow!35} 0.837 & 0.193 & 49.31 & 172 
%         & 29.83 & 0.903 & \cellcolor{red!35}{0.248} & 75.91 & 124 \\
%         Compact-3DGS
%         & 27.08 & 0.798 & 0.246 & 48.88 & 135 
%         & 23.32 & 0.831 & 0.202 & 39.40 & 201 
%         & 29.83 & 0.901 & 0.257 & 42.91 & 191 \\
%         C3DGS
%         & \cellcolor{yellow!35} 27.15 & 0.801 & 0.241 & \cellcolor{yellow!35} 29.28 & 131 
%         & 23.47 & \cellcolor{orange!35} 0.838 & \cellcolor{yellow!35} 0.188 & \cellcolor{yellow!35} 18.42 & 211 
%         & 29.40 & 0.898 & \cellcolor{yellow!35} 0.255 & \cellcolor{yellow!35} 25.07 & 156 \\
%         LightGaussian
%         & 26.93 & 0.800 & 0.244 & 51.13 & \cellcolor{red!35}{216} 
%         & 23.32 & 0.830 & 0.204 & 30.03 & \cellcolor{red!35}{374}
%         & 29.09 & 0.894 & 0.262 & 45.42 & \cellcolor{red!35}{286} \\
%         EAGLES
%         & 27.13 & \cellcolor{orange!35} 0.805 & \cellcolor{yellow!35} 0.239 & 71.30 & \cellcolor{yellow!35} 148 
%         & \cellcolor{yellow!35} 23.48 & 0.836 & 0.200 & 35.33 & \cellcolor{orange!35} 265 
%         & \cellcolor{yellow!35} 29.89 & \cellcolor{red!35}{0.906} & \cellcolor{orange!35} 0.249 & 64.31 & 169 \\
%         HAC
%         & \cellcolor{red!35} 27.43 & 0.\cellcolor{yellow!35} 804 & 0.242 & \cellcolor{orange!35}{16.00} & 106 
%         & \cellcolor{red!35}{24.16} & \cellcolor{red!35} 0.846 & \cellcolor{orange!35} 0.187 &  \cellcolor{red!35}{8.35} & 134 
%         & \cellcolor{orange!35} 29.97 & \cellcolor{yellow!35} 0.903 & 0.267 &  \cellcolor{red!35}{4.78} & \cellcolor{orange!35} 238 \\
%         \midrule
%         Ours-Sparse
%         & \cellcolor{orange!35} 27.33 & \cellcolor{red!35}{0.807} & \cellcolor{red!35} 0.237 & \cellcolor{red!35} 14.84 & \cellcolor{orange!35} 193 
%         & \cellcolor{orange!35} 23.80 & \cellcolor{red!35} 0.846 & \cellcolor{red!35} 0.182 & \cellcolor{orange!35} 13.17 & \cellcolor{yellow!35} 236
%         & \cellcolor{red!35}{30.16} & \cellcolor{orange!35}{0.905} & \cellcolor{orange!35} 0.249 & \cellcolor{orange!35} 15.71 & \cellcolor{yellow!35} 213 \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

